Graph Neural Tangent Kernel: Fusing Graph Neural Networks with Graph Kernels

While graph kernels (GKs) are easy to train and enjoy provable theoretical guarantees, their practical performances are limited by their expressive power, as the kernel function often depends on hand-crafted combinatorial features of graphs. Compared to graph kernels, graph neural networks (GNNs) usually achieve better practical performance, as GNNs use multi-layer architectures and non-linear activation functions to extract high-order information of graphs as features. However, due to the large number of hyper-parameters and the non-convex nature of the training procedure, GNNs are harder to train. Theoretical guarantees of GNNs are also not well-understood. Furthermore, the expressive power of GNNs scales with the number of parameters, and thus it is hard to exploit the full power of GNNs when computing resources are limited. The current paper presents a new class of graph kernels, Graph Neural Tangent Kernels (GNTKs), which correspond to infinitely wide multi-layer GNNs trained by gradient descent. GNTKs enjoy the full expressive power of GNNs and inherit advantages of GKs. Theoretically, we show GNTKs provably learn a class of smooth functions on graphs. Empirically, we test GNTKs on graph classification datasets and show they achieve strong performance.

==> gen_proof.tex <==
\subsection{Kernel Linear Regression}

We consider a kernel linear regression problem. Define $\vect{x}_i \mapsto \Phi(\vect{x}_i)$ as the feature mapping induced by our GNTKs. This maps each input graph $\graph_i, \forall i \in [n]$ to a potentially high dimension space $\Phi(\vect{x}_i) \in \cH$. In kernel linear regression, we wish to learn a function of the form $f_{ker}(\vect{x}_i) = \vect{w}^\top \Phi(\vect{x}_i)$ where $\vect{w}$ is a solution of following optimization problem:
\begin{align*}
\min \quad & \norm{\vect{w}}_2 \\
\text{s.t.} \quad &  \vect{w}^\top \Phi(\vect{x}_i) = y_i, \quad \forall i \in [n].
\end{align*}
The solution of this problem is given by $\vect{w} =\mat{\Phi}(\mat{\Phi}^T \mat{\Phi})^{-1}\vect{y}$, where $\mat{\Phi}$ is a $n$-column matrix with each column consists of the feature mapping of data point $\vect{x}_i$. The norm $\vect{w}$ is given by
$\norm{\vect{w}}_\cH = \sqrt{\vect{y}^\top (\mat{\Phi}^\top \mat{\Phi})^{-1} \vect{y}}$.

\subsection{Rademacher Complexity of Kernel-Based Hypotheses}
% reference: https://cs.nyu.edu/~mohri/mls/lecture_5.pdf
Let $K(\cdot, \cdot): X\times X \rightarrow \mathbb{R}$ be a positive definite kernel and $\Phi(\cdot): X \rightarrow \mathcal{H}$ be the feature mapping induced by kernel $K$. The hypothesis class 
\begin{align*}
\mathcal{F}_B = \{\vect{x} \mapsto \vect{w}^\top \Phi(\vect{x}): \norm{\vect{w}}_{\cH} \le B \}
\end{align*}
has the empirical Rademacher complexity 
\begin{align*}
\cR_S(\cF_B) & = \frac{1}{n}\E_{\vect{\epsilon} \in \{\pm 1\}^n}
\left[\sup_{f\in\cF_B} \sum_{i=1}^n \epsilon_i f(\vect{x}_i)\right] \\
& \le \frac{B\sqrt{\tr[\mat{K}]}}{n}.
\end{align*}
To prove the above statement, we have
\begin{align*}
\cR_S(\cF_B) & = \frac{1}{n} \E_{\vect{\epsilon}} \left[ \sup_{\norm{\vect{w}}_\cH \le B} \vect{w}^\top \left(\sum_{i=1}^n \epsilon_i  \Phi(\vect{x}_i) \right)\right] \\
& \le \frac{B}{n} \E_{\vect{\epsilon}} \left[ \norm{\sum_{i=1}^n \epsilon_i  \Phi(\vect{x}_i)} \right] \\
& \le \frac{B}{n} \sqrt{\E_{\vect{\epsilon}} \left[ \norm{\sum_{i=1}^n \epsilon_i  \Phi(\vect{x}_i)}^2 \right]} \\ % by Jensen's inequality
& \le \frac{B}{n} \sqrt{\E_{\vect{\epsilon}} \left[\sum_{i=1}^n  \norm{\Phi(\vect{x}_i)}^2 \right]} \\
& = \frac{B\sqrt{\tr(\mat{K})}}{n} .
\end{align*}
Therefore, the empirical Rademacher complexity is bounded by a constant related to the norm of the coefficient $\vect{w}$ and the trace of kernel $\tr(\mat{K})$.

\subsection{Generalization Bounds for Kernel Linear Regression}
From the theory of of Rademacher complexity, we have the following theorem:
\begin{thm}\label{thm:rademacher_gen}
Suppose the loss function $\ell(\cdot, \cdot)$ is bounded in $[0,c]$ and is $\rho$-Lipschitz in the first argument. Then with probability at least $1-\delta$ over sample $S$ of size $n$:
\begin{align*}
\sup_{f\in \cF} \{L_{\cD}(f) - L_S(f) \} \le 2 \rho \cR_S(\cF) + 3c \sqrt{\frac{\log(2/\delta)}{2n}}
\end{align*}
\end{thm}
A proof of this theorem can be found in the appendix of \cite{arora2019fine}. With the ingredients provided above, we are now ready to prove Theorem~\ref{thm:kernel_gen}.

For a kernel linear regression problem with kernel matrix $\mat{\Theta}$ and label $\vect{y}$, the optimal solution satisfies the bound $\norm{\vect{w}} \le \sqrt{\vect{y}^\top \mat{\Theta}^{-1} \vect{y}}$. We can also know that the Rademacher complexity of the corresponded hypothesis class is bounded by $\frac{\sqrt{\vect{y}^\top \mat{\Theta}^{-1} \vect{y} \tr(\mat{K})}}{n}$.
Since the loss function is $1$-Lipschitz, combined with Theorem~\ref{thm:rademacher_gen}, we conclude the generalization bound for kernel linear regression satisfies
\begin{align*}
L_{\cD}\left(f_{ker}\right) \le 2\frac{\sqrt{\vect{y}^\top \mat{\Theta}^{-1}\vect{y}\tr\left(\mat{\Theta}\right)}}{n} + 3c \sqrt{\frac{\log(2/\delta)}{2n}}.
\end{align*}



==> rel.tex <==
%Graph Data

%Graph Kernels

%GNNs



